The American Sign Language Knowledge Graph: Infusing ASL Models with Linguistic Knowledge

Language models for American Sign Language (ASL) could make language technologies substantially more accessible to those who sign. To train models on tasks such as isolated sign recognition (ISR) and ASL-to-English translation, datasets provide annotated video examples of ASL signs. To facilitate the generalizability and explainability of these models, we introduce the American Sign Language Knowledge Graph (ASLKG), compiled from twelve sources of expert linguistic knowledge. We use the ASLKG to train neuro-symbolic models for 3 ASL understanding tasks, achieving accuracies of 91% on ISR, 14% for predicting the semantic features of unseen signs, and 36% for classifying the topic of Youtube-ASL videos.

==> sections_draft1/1_intro.tex <==
% The problem: the lexicon is constantly changing, and real-world systems will need to adapt to these changes. For example telephone, computer.
Historically, the ASL lexicon has expanded through processes such as lexicalization, localization, ...

The appearance and meaning of signs is highly structured and particularly helpful in learning tasks/skills related to understanding a dynamic lexicon

Knowledge graphs provide an opportunity to integrate reliable representations of these linguistic priors into neural models.

Knowledge-infused and neuro-symbolic learning. 

In this work, we...

==> sections_draft1/2_bg.tex <==
\subsection{Knowledge Graph Construction}
Knowledge graphs bring together a variety of facts and structure them such that knowledge pertaining to a particular topic may be easily accessed and used to train neuro-symbolic models (Wang). The structure facts are represented as triples of the form <subject entity, relation, object entity> such that the entities represent concepts and the relations represent predicates, as in \todo{Example} (Wang, Xue). Knowledge graphs can be described using ontologies/schemas, which are created by defining classes and relations (Ryen/Heist).

Due to their unique structure, knowledge graphs can be used in unique ways. \todo{“Knowledge from a knowledge graph can be exploited using deductive and inductive approaches (Ryen). Deductive approaches concern extracting knowledge using entailment and reasoning through logical axioms and rules. Inductive approaches concern deriving knowledge through analyzing patterns in a knowledge graph. ” } Knowledge graph embeddings are a popular, data-driven approach to representing inferences. \todo{“In embedding, components of a knowledge graph are embedded into continuous vector space, a transformation which “simplifies manipulation while preserving the inherent structure of the knowledge graph” }(Ryen, Wang). The embedding can be used for various tasks such as knowledge graph completion, relation extraction, entity classification, and entity resolution, as well as training machine learning models for classification, regression, and recommendation. (Ryen, Wang)” Knowledge graphs are a versatile [and WHAT??] way of storing data because they allow information to be connected in various unique ways. 

\todo{Knowledge graphs can be created through manual curation, creation from unstructured sources (such as free text), or from structured or semistructured sources (Heist). To integrate data from semi-structured sources into knowledge graphs, [WE????] must create ontologies by “defining concepts and relations through domain analysis or analyzing available data” then preprocess data including “enrichment (adding additional information to data), reconciliation (matching entities from different sources), and cleaning (improve the quality of data)” (Ryen). The next task is to integrate the data, or to convert it from its source style to the knowledge graph format (Ryen). Data can be integrated through manually defining entities based on the source, or by mapping directly from the source (often done for tabular data)  or mapping through a series of statements defining how data is to be mapped from its source (Ryen). Mapping is standardized by W3C (Ryen). A knowledge graph can hold and connect data from several different sources. Knowledge graph data is evaluated with “five widely used indicators: accuracy (whether data reflects the facts correctly), consistency (data agree with each other), completeness (whether data contains all relevant data of interest), timeliness (whether data is up to data) and redundancy (dataset does not contain two identical objects” (Xue).}


\subsection{Word Form and Meaning in Sign Languages}
The present investigation focuses specifically on American Sign Language (ASL), a sign language used by communities in the United States and Canada.
Sign languages are complete and natural languages primarily used by deaf and hard-of-hearing people. Sign languages and spoken languages are similar in many ways: there are over one hundred sign languages used by different communities around the world \todo{[eberhard2023]}; and sign languages demonstrate full phonological, lexical, and syntactic complexity \todo{[e.g., padden2016; liddell1980?; padden2001; coulter2014]}. Despite these broad similarities, sign languages also differ from spoken languages in ways which may present unique challenges for the application of NLP. Despite tens of millions of signers around the world, there is a dearth of high-quality lexical datasets that could support the training of machine learning models. Additionally, sign languages are visual languages and typically do not have any widely-used written form, which necessitates the use of video-based parsing and recognition rather than acoustic or textual recognition. 

The phoneme is the smallest unit of language--in spoken languages, these are sometimes referred to as "speech sounds". In ASL, signs are distinguished from each other phonologically based on the shape, orientation, movement, and location of the signer's hands as well as nonmanual markers (such as lip shape and eyebrow height) \todo{[herrmann2011; michael2011]}. Understanding the phonological structure of the language has direct implications for training NLP: for example, Kezar (2023) achieved a 9 percent improvement in isolated sign recognition accuracy by including auxiliary predictions of signs' phonological features. Phonemes are not generally considered to carry any particular meaning, but rather but rather are the inventory of building blocks of forms that can be combined to create words or signs. 

The role of meaning is typically considered to be limited to higher levels of lexical representation, such as morphemes and words. For over a century, the prevailing linguistic theory has asserted that words and morphemes are arbitrary symbols for meaning (Saussare 1916, others). The theory of arbitrariness can be compared with \textit{systematicity}: the theory that within lexicons, there are consistent relationships between the production and meaning of words. For example, in the word "millipede", \textit{milli-} can be observed in million, and the sounds in \textit{-pede} can be observed in other words referring to feet (pedometer, pedestrian, and tripod). 

Linguists have generally approached this debate in a top-down manner by identifying a potential phonological property that carries consistent meaning, and then searching for evidence that it does so. For example, Hutchins (1998) identifies 46 English phonesthemes–-sound clusters that tend to carry a particular meaning (e.g., the sound /gr-/ is associated with deep-toned, threatening noises, as in \textit{growl}, \textit{gruff}, \textit{grunt}, and \textit{grunt}).

In American Sign Language, Börstell et al. (2016) observed that signs for concepts that inherently include multiple entities (e.g., eyes, shoes, family) are frequently denoted by two-handed signs. Similarly, Occhino (2017) examined signs in ASL and Libras (Brazilian Sign Language) that used a claw handshape and found that across both languages, convex/concave shapes (such as \href{https://asl-lex.org/visualization/?sign=ball}{BALL} or \href{https://asl-lex.org/visualization/?sign=bowl}{BOWL} in ASL) were frequently denoted by signs using a claw handshape.

%[Idk how I feel about this next paragraph.]
Understanding arbitrariness and systematicity within lexica has important implications for how we approach the task of word recognition: if words with similar forms have similar meanings, then to achieve high accuracy on word recognition tasks, humans (and their NLP counterparts) must have high perceptual precision. Under this scenario, in the case of machine translation (for example), broader linguistic context (at the sentence or discourse level) is unlikely to help guess the correct word. This is because words with similar meanings, which could appear in similar contexts, are likely to be phonologically and perceptually similar to one another. On the other hand, when languages have a high degree of systematicity, this might suggest that for tasks like sentiment analysis or identifying textual themes, encoding the exact phonological representation of words may not be necessary. Even if there are slight errors in phonological features, relevant semantic information can still be extracted, allowing for a rough understanding of the meaning.

==> sections_draft1/3_overview.tex <==
% \input{tables/sources}
% \input{tables/relation_types}
% \input{tables/stats}

\subsection{Sources}
We include eight diverse, expert-curated sources of knowledge in ASLKG. The sources were selected based on their linguistic content. We outline the key features of each source below.

\textbf{ASL-LEX} is a lexical database for American Sign Language containing phonological properties for 2732 signs. The data was collected from published databases, an ASL vocabulary test, and in-house psycholinguistic experiments. ASL-LEX contributes reliable phonological information to the knowledge graph. 
% Example: <‘since’, Phonological\(_\)Complexity, 2.0> 

\textbf{ASLLRP Sign Bank} is a database of linguistically annotated videos of native signers of ASL, containing 41,830 examples of lexical signs. The data were collected from native signers producing citation-from signs and continuous signing. ASLLRP contributes reliable phonological information to the knowledge graph.  
% Example: < ‘tiptoe’, Dominant\(_\)Start\(_\)Handshape, ‘bent-1’> 

\textbf{Lancaster Sensorimotor Norms} provides association strengths between 39,707 concepts and six perceptual modalities and five action affectors. It was collected from 3,500 participants through surveys. Lancaster Sensorimotor Norms contributes information about semantic associations with the body, which are iconically represented through effectors (for example, the word ‘food’ is associated with the mouth).  
Examples: <‘nervous’, Interoceptive.mean, 4.053> , <‘nervous’, Olfactory.mean, 0.053> 

\textbf{Linguistic Inquiry and Word Count (LIWC)} is a dataset from a text analysis program that counts words in 22 psychologically meaningful categories. The data was collected from text samples from studies. LIWC contributes information about semantic associations to the knowledge graph.
Example: < ‘individual’, D-Inspired, 0.166> 

\textbf{Empath} provides lexical categories in the same format as LIWC, but across \todo{200} categories generated by a semi-supervised model trained on data from fiction. Empath contributes information about semantic associations to the knowledge graph. 
Example: <‘puppet’, M-toy, 1.0

\textbf{Iconicity} is a database of signs annotated according to various parameters of iconicity, such as personification or the presence of iconic location and movement. The data were collected from an online sign language dictionary. Iconicity describes the relationship between form and meaning, and these facts provide context to \todo{[WHAT]}

\textbf{Semantic Associations} \todo{[summary]} Example: < ‘staff’, response, ‘dormitory’>

For further details about each of these sources, see \ref{tab:graph_sources} \todo{[Link should have different name]}
Each $\fact{} \in \facts$ is labeled with its source.



\subsection{Structure}
The ASLKG $\graph$ is a set of entities $\entities$ interconnected by a set of relations $\relations$ according to a set of facts $\facts$ pertaining to ASL signs:
\begin{align}
    \graph &:= \langle \entities, \relations, \facts \rangle \\
    \entities &:= \{ \entity{1}, \entity{2}, \dots \entity{E} \}, \entity{i} \in \mathbb{Z} \\
    \relations &:= \{ \rel{1}, \rel{2}, \dots \rel{R} \}, \rel{j} \in \mathbb{Z} \\
    \facts &:= \{ \fact{1}, \fact{2}, \dots \fact{F} \}, \\
    \fact{k} &:= (h,r,t) \hspace{0.5em} \quad \hspace{0.5em} h,r \in \entities, \hspace{0.6em} r \in \relations
\end{align}
All head entities $h_k$ represent a sign and all tail entities $t_k$ represent either another sign or some real number (e.g. $(\texttt{}, \texttt{}, \texttt{})$

\paragraph{Relation Types.} 
To enable more targeted applications of the ASLKG (see \ref{sec:overview_applications}), we partition $\relations$, and by extension $\facts$, according to the type of knowledge each $\rel{k}$ conveys about its subject $h_k$. 
See Table~\ref{tab:relation_types} for a description of each relation type.\footnote{Note that some types, such as \texttt{phonetic} and \texttt{morphological}, do not have many relations due to the availability of relevant knowledge bases on the internet. Future versions of the ASLKG may expand these relation types.}
\begin{align}
    \types &:= \{ \small \texttt{phonetic}, \texttt{phonological}, \dots \} \\
    \text{type} &: \relations \cup \facts \rightarrow \types \\
    \reltype{k} &:= \facttype{k}, \quad \forall \rel{k} \in \relations \\
    \relationstype{t} &:= \{~\rel{i}~|~\reltype{i} = t, \rel{i}\in\relations~\} \\
    \factstype{t} &:= \{~\fact{i}~|~\facttype{i} = t, \fact{i}\in\facts~\} \\
    \text{s.t.}& \hspace{0.5em} \bigcup_{\text{t} \in \types} \factstype{t} = \facts \hspace{0.5em} \land \hspace{0.5em} \bigcap_{\text{t} \in \types} \factstype{t} = \emptyset
\end{align}

\paragraph{Cross-fold Validation.} For uses of the ASLKG requiring train, validation, and test splits of the set of head , such as triple verification

\input{tables/sources}

\input{tables/stats}

\subsection{Applications} \label{sec:overview_applications}
Structured knowledge enables

\subsection{Ethical Considerations and Limitations}

==> sections_draft1/4_experiments.tex <==
The intended use of the ASLKG is to provide new, neuro-symbolic methods of processing and representing ASL video data.
In this section, we define a set KG-oriented tasks and neuro-symbolic models that experimentally verify the ASLKG's utility for ASL understanding.
We organize these tasks and models into three groups, derived from the \textit{knowledge-infused learning} framework: shallow, semi-deep, and deep knowledge infusion. \todo{CITE}
The overarching goal of knowledge-infused learning is to translate task-specific knowledge into a model's parametric space, usually through graphical and neural mechanisms.

\textit{Shallow} knowledge infusion seeks to contextualize training examples with expert knowledge, e.g. the compositional nature of signs.
We consider this class of methods ``shallow'' because the contextualization usually applies to a model's input or output only, hence it is unclear to what extent that knowledge permeates through the model's parameters.

\textit{Semi-deep} knowledge infusion seeks to embed expert knowledge into the parametric space.
We consider this class of methods to be ``semi-deep'' because the knowledge, now represented as floating-point vectors, 

Recognizing that ASLKG facts $\facts$ predominantly represent the linguistic nature of ASL signs, we call our methodology \textit{linguistic knowledge infusion}.

\subsection{Shallow Knowledge Infusion}
 - natural language description
 - algebraic definition: function

 - Exact:FGM
 - Neural: End-to-end
 - Non-parametric: Nearest Neighbor

\subsection{Semi-Deep Knowledge Infusion}
 - natural language description
 - algebraic definition: function

 - KG node embeddings
    - purpose
    - algorithms
    - isr models
    
 - Semantic Backoff
    - purpose

\subsection{Deep Knowledge Infusion}
 - natural language description
 - algebraic definition: function

 - Task/data: Youtube ASL Topic Prediction
 - Topic creation
 - Sliding window phonologizer
 - sign recognition
 - Embedding
 - Topic recognition

==> sections_draft1/5_results.tex <==


\input{tables/phon2sign}

\input{tables/semantic_prediction}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/sempred.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure*}

\input{tables/isr_results}

==> sections_draft1/6_discussion.tex <==

Shallow


Semi-Deep

 - 
 - error correction

Deep
